Multi-Variant Execution of Parallel Programs

Multi-Variant Execution Environments (MVEEs) are a promising technique to protect software against memory corruption attacks. They transparently execute multiple, diversified variants (often referred to as replicae) of the software receiving the same inputs. By enforcing and monitoring the lock-step execution of the replicae's system calls, and by deploying diversity techniques that prevent an attacker from simultaneously compromising multiple replicae, MVEEs can block attacks before they succeed. Existing MVEEs cannot handle non-trivial multi-threaded programs because their undeterministic behavior introduces benign system call inconsistencies in the replicae, which trigger false positive detections and deadlocks in the MVEEs. This paper for the first time extends the generality of MVEEs to protect multi-threaded software by means of secure and efficient synchronization replication agents. On the PARSEC 2.1 parallel benchmarks running with four worker threads, our prototype MVEE incurs a run-time overhead of only 1.32x.

==> ack.tex <==
% Dit was voor IEEE
% \section*{Acknowledgement}

\begin{acks}
The authors want to thank the Agency for Innovation by Science and Technology in
Flanders (IWT), the Fund for Scientific Research - Flanders, and Ghent
University for their support. 
\todo{PER: Anyone you need to acknowledge here?}
\end{acks}


==> background.tex <==
\section{Background}
\label{Background}

\subsection{Multi-Variant Execution}

\begin{figure}
\centering \includegraphics[width=6cm]{basic_operation.pdf}
\caption{Basic operation of a MVEE}
\label{GHUMVEE_Basic1}
\end{figure}

Rather than launching an application directly, a user seeking protection against
ROP and other memory-based attacks will invoke the MVEE's monitor to replicate
the application.  Upon invocation, the monitor launches two or more replicae of
the application, attaches itself to those replicae using the operating system's
debugging API, and feeds them their original arguments. The monitor is
responsible for ensuring that the replication is transparent, i.e., that with
the exception of timing, the replication does not influence the I/O behavior of
the application as observed by the user. To that end, the monitor intercepts all
I/O between the replicae and their environment. Fig.~\ref{GHUMVEE_Basic1}
illustrates this for two system calls, \code{brk} and \code{write}. For a call
like \code{brk}, the monitor waits until both replica have issued the call
before passing them through to the kernel to allocate memory for both
replicae. After the kernel has processed the system calls, the monitor passes
the resulting pointers back to the replicae. Of the two \code{write} calls by
the two replicae, the monitor passes only one to the kernel, as the external
world should observe only one write operation.

The result of the call is then replicated by the monitor and passed to both
replicae, at which point they continue executing. During the replicae's
execution, the monitor checks their I/O to ensure that they behave
identically. Whenever an I/O divergence is detected among the replicae, the
monitor signals this and halts execution before the I/O operation is passed on
to the environment. For that reason, the replicae are synchronized at all I/O
operations they initiate, as shown in Fig.~\ref{GHUMVEE_Basic1}. For monitoring
and replicating the I/O of the replicae, the monitor can use either the
\code{ptrace} or the \code{process\_vm\_*} Linux APIs.


